Logic Blog 2022

The 2022 logic blog has concentrated on the connections of group theory and logic. It discusses Gardam's 2021 refutation of the Higman/ Kaplansky unit conjecture, and its connections to logic and to computation. The rest is about topological groups of various kinds, in particular a computational theory of tdlc groups, and a duality between locally Roelcke precompact groups and certain countable structures called meet groupoids.

==> sections2022/Lam_Nies.tex <==
 \section{Lam and Nies: Whitehead's problem and the category of sets}
  SET is the category of sets with maps in between them.  Ka Ho Lam, a former student of Nies, asked whether there are  properties of this category that are not decided by ZFC. Here we sketch how to obtain  such a property,  which is first order in the language of SET. As an additional bonus it is invariant under equivalence of categories due to MacLane, as recalled below. This means that they are natural properties from the point of view of categories.  Semantically speaking, what we prove is that  there are two countable models of ZFC such that their categories of sets are not equivalent.

 

  An abelian group $A$  is called a \emph{Whitehead group} if   each extension of $A$ by $\ZZ$ is splitting. This means that for each exact sequence $0 \to \ZZ \to E \to A \to 0$, there is a morphism $A \to E$ inverting $E \to A$. Clearly each free group is a Whitehead group. 
 The Whitehead problem asked whether the converse holds. Shelah~\cite{Shelah:74,Shelah:75},  proved that this statement  is independent of ZFC. If $V=L$ then the conjecture holds. If $MA \lland \lnot CH$ then there is a Whitehead group that is not free. 
 Also see   \cite{Shelah:77} which shows that the problem can have a negative answer even in the presence of CH. We note that the counterexamples are necessarily uncountable. 

  To obtain a sentence in the language of the category of sets which ZFC cannot decide, we first-order  interpret the category of abelian groups in the category of sets. The sentence is invariant under equivalence of categories.  
  
  Another way to obtain such a sentence would be to express the generalized continuum hypothesis GCH in the category of sets. (However, it is less clear that the resulting sentence is invariant.) We need a subobject classifier $\Omega$, namely a 2-element set, and want to talk about monomorphisms  $\aaa\colon U \to \mathrm{Mor}(X,\Omega)$, which express  subsets of $\+ P(X)$.  We need to replace these by maps $\overline \aaa \colon U \times X \to \Omega$ and somehow need to express that $\aaa$ is a  monomorphism   via a category theoretic property of $\ol \aaa$.
  \subsection{Background on categories, and first-order logic}
 
  We view categories as generalised structures where the domain can be a class (consisting of the morphisms); they only have  a ternary relation $R$ for composition of morphisms. $Rfgh$ means that $fg$ is defined and equals $h$; henceforth, we will write this as $fg= h$. A morphism $f$ is an identity morphism if $ff=f$. Formally speaking, objects are identified with the corresponding  identity morphisms, so we don't need a special sort for them. However, in practice we use the usual letters $A,B,C, \ldots$ for them, and   write $1_A$ if we want to view $A$ as morphism,  e.g., in writing things like $ 1_A f =f$. Given a category, there are first-order definable  functions $\sss$ and $\tau$    that assign  to a morphism its source and target objects, respectively. We have 
  \bc $\sss(f)= h$ if $hh= h \land hf=f$ and $\tau(f)= \ell$ if $\ell \ell = \ell \land f\ell=f$. \ec We write \bc $\mor f A B $ for $\sss(f) = A \land \tau(f)= B$. \ec We sweep under the rug some  logical complications that ensue because   the domain of the ``structure" usually is a proper class. Merely  note that saying that a subclass, or a  function,  is first-order definable by such and such formula   means that ZFC proves the equivalence of the original definition  of the function (which was given in the usual  the language of set theory) with what the defining formula (which is in the language of the category) expresses.
  
   Two categories $\+  C, \+ D$ are \emph{equivalent} (in the sense of MacLane) if there is a functor $T\colon \+ C \to \+ D$ which is 
  
 \bi \item  full and faithful, i.e. for any two objects $A, B$ of $\+ C$, the map \bc $\mathrm{Hom}(A,B) \to \mathrm{Hom} (TA,TB)$ \ec   induced by $T$ is surjective and injective;
  
 
\item essentially surjective (or dense), i.e.   each object $B $ in $\+ D$ is isomorphic to an object of the form $TA$, for some object $A$ in $\+ C $. \ei
  
Freyd~\cite{Freyd:76} (also see   \href{http://angg.twu.net/Freyd76.html}{this site})     characterised the properties of categories  that are invariant under equivalence.
 These are the ones that  are   diagrammatic  (essentially: defined in a language of diagrams and using  the   quantifiers $\forall, \exists$).  
  
   \subsection{A statement about SET that is  undecidable in ZF, and invariant under equivalence of categories}
    In ZF  it is much easier to obtain an invariant  sentence in the language of SET that cannot be decided. 
We say that a \emph{category} satisfies the axiom of choice   if each epimorphism has a right inverse. That is, if $\mor f A  B$ is an epimorphism  then there is $\mor g B A$ such that $gf=1_B$.  It is well known that in ZF, the axiom of choice for SET is equivalent to the usual axiom of choice. The only extra trouble is due to the fact that we want the property to be invariant under equivalence. The next two lemmas check this.

\begin{claim} Let $T \colon \+ C \to \+ D$ be an equivalence of categories. Suppose that  $\mor f A  B$ is  a morphism  in $\+ C$. Then \bc  $f$ is an epimorphism in $\+ C$  $\LR$  $T(f) $ is an epimorphism in $\+ D$. \ec \end{claim}
\begin{proof} \rapf Suppose $\mor {\wt g_i} {T(B)} {\wt C}$ in $\+ D$ for $i=0,1$, and $T(f)\wt g_0= T(f)\wt g_1$. Since $T$ is dense, there is an object  $C \in \+ C$ and an isomorphism $\mor p  {\wt C} {T(C)}$.  Since $T$ is full, there are $\mor {g_i} B C$ in $\+ C$ such that $T(g_i)= \wt g_i p$. Since $fg_0= fg_1$ we have $ g_0= g_1$, and hence $\wt g_0= \wt g_1$. 

\lapf This implication   holds for any faithful functor. 

 \end{proof}
\begin{fact} Let $\+C, \+ D$ be equivalent categories. Then \bc  $\+ C$ satisfies the axiom of choice $\LR$  $\+ D$ satisfies the axiom of choice. \ec \end{fact}
\begin{proof} Since $T$ has an inverse that is also an equivalence of categories, we only need to show $\LA$. So suppose $\mor f A B$ is an epimorphism  in $\+ C$. Then in $\+ D$ there is  $\mor {\wt g} {T(B)} {T(A)}$ such that $\wt g T(f)= 1_{T(B)}$. Since $T$ is full, $\wt g = T(g)$ for some $\mor g BA$. Then  $gf=1_B$ since $T$ is faithful. \end{proof}

  
  \subsection{The category $Ab$} 
 
 Recall that an abelian group $A$ is free if and only if  it is projective: for any epimorphism $\mor g UV$ and any morphism $\mor h AV$ there is $\mor f AU$ such that $fg = h$. For the easier direction, if $A$ is freely generated by a set $X$, let $f(x)$ for $x \in X$ be a preimage of $h(x)$ in $U$, and extend. The point of replacing free by projective is that being projective is first-order definable via diagrams.
 
%  \begin{prop} Being projective is first-order definable in a category. \end{prop}
%
%\begin{proof}  Let  $\mathcal{S}$ be  the predicate which states that $f$ is an epimorphism, defined as $$\mathcal{S}(f)\Leftrightarrow\forall a\forall b( fa =  fb\rightarrow a=b).$$ An object $G$ is projective iff $$\forall f\forall g(\mathcal{S}(f)\wedge t(f)=G\wedge t(g)=G\rightarrow\exists h(s(h)=s(g)\wedge t(h)=s(f)\wedge  hf=g)),$$  \end{proof}
 
 
\begin{prop} The class of Whitehead  groups  is first-order definable in the  category     $Ab$ (over ZFC). \end{prop} 
\begin{proof}
%Some care is needed when formulating exact sequences.    This might be  a first-order property of diagrams $N\stackrel f \to A  \stackrel g \to Q$, so in effect of a 5-tuple.  If it doesn't work in general one  can still do it for 
 
1.  We can  define what it means that $f=0$ for $\mor f AB$: this holds exactly when $f g_0= fg_1$ for each $B$ and each pair of morphisms $\mor {g_i} A B$. 
 
2.   $\ZZ$ (up to isomorphism)  is the only  projective object not isomorphic to a proper direct product. 

3. A sequence $ \ZZ\stackrel f \to A  \stackrel g \to Q$ is exact exactly if  the monomorphism $\mor f \ZZ A $ is maximal such that $fg =0$; that is, if  there is a proper monomorphism $\mor h \ZZ  M$ and monomorphism $\mor {\wt f} M A$ such that $f = h \wt f$, then $\wt f g \neq 0$.  \end{proof}

So there is  a first-order  sentence $\theta$   in the language of $Ab$ expressing  that some  Whitehead group   is not projective. 

%
%\begin{prop} Check what  happened to that diagrammatic language in the meantime. Newer references, better ways to do it, formal notation for  it. \end{prop}
\begin{prop} The   statement $\theta$ is   preserved under equivalence of categories  in the sense of MacLane. \end{prop} 
This is because the definitions are   diagrammatic in the sense of Freyd as discussed above.
We   conclude that the first-order theory of $Ab$ is not determined by ZFC, and that there are two countable models of ZFC such that their categories $Ab$ are not equivalent.

 
 \subsection{The category $SET$}
For  first-order interpretations see e.g.\ Hodges, Model theory, Ch.\ 5, or Tent-Ziegler, Model theory. One can  then formulate the notion of diagrammatic interpretations. It means the f.o.\ properties are given by diagrams a la Freyd. 


\begin{prop}  There is a diagrammatic interpretations of the category $Ab$ in the category $SET$. \end{prop} 

\begin{proof}
%	\andre{don't use $G'$ that's the commutator group}
%	Let the category of free abelian groups with group homomorphisms be $\mathcal{F}$.\\
%	Given an abelian group $G$, there is a free abelian group $G'$ generated by the elements of $G$. We have a canonical epimorphism $f_G:G'\rightarrow G$ which maps an element of $G'$ to the sum of its components. Let the kernel of $f_G$ be $G''$ and the corresponding monomorphism be $g_G:G''\rightarrow G'$. $G$ is the cokernel of $g_G$. Notice that a group homomorphism between free abelian groups is a monomorphism in $Ab$ if and only if it is a monomorphism in $\mathcal{F}$. We can represent an abelian group $G$ by using the triple $(G'',G,g_G)$ where $g_G:G''\rightarrow G'$ is a monomorphism in $\mathcal{F}$.\\
%	Consider abelian groups $A,B$ and a group homomorphism $h:A\rightarrow B$. By the universal property of free abelian groups, there is an induced group homomorphism $h':A\rightarrow B'$ such that $h'\circ f_b=h$. Repeating this process to $f_A\circ h'$, we have the following commutative diagram
%	$$
%\begin{tikzcd}
%A''\ar[r]\ar[d,"g_A"]& B''\ar[d,"g_B"]\\
%A'\ar[r,"f_A\circ h'"]\ar[d,"f_A"]& B'\ar[d,"f_B"]\\
%A\ar[r,"h"]& B
%\end{tikzcd}
%$$
%Thus, all morphisms in $Ab$ can be represented by the commutative diagrams of the following form
%$$
%\begin{tikzcd}
%A''\ar[r]\ar[d,"g_A"]& B''\ar[d,"g_B"]\\
%A'\ar[r]& B'
%\end{tikzcd}
%$$
%This interprets $Ab$ into $\mathcal{F}$.\\ 
%
%\andre{How do you interpret $\+ F$ in SET? }
%\andre{You need to define what f.o.\ interpretation means for categories, and discuss it, compare to Hodges}
An object (abelian group)  is represented by a tuple of elements of SET \bc  $A, S, p_0, p_1,  f,g, m, sw$ \ec   where  $A, S$ are objects, $f \colon S \to A$ represents  the binary  group operation, $g \colon A\to A$ is the inverse, $m \colon 0 \to A$, $p_i \colon S \to A$ are the projections. One can say  in a first-order way via diagrams that $S$ has the universal property of $A \times A$. One can formulate the abelian group axioms via diagrams, similar to the stuff on Hopf algebra in \href{https://www.cs.auckland.ac.nz/~nies/Students/Dominik_Roje_Honours_Dissertation.pdf}{Dominik Roje's Honours thesis} page 19. For commutativity,  one needs to require the morphism \bc $sw \colon S \to S$ \ec  that switches the components. 

A morphism $f \colon A\to B$ is then just a set morphism that satisfies some ``commuting diagram property" expressing that it preserves the group operations.  	
\end{proof}

\begin{prop} If there is a diagrammatic    interpretation $\Gamma$ of $\+ C_0$ in $\+D_0$, and $\+ D_0 $ is MacLane equivalent to $\+ D_1$ then the category $\+ C_1$ obtained as $\Gamma(\+ D_1)$ is MacLane equivalent to $\+ C_0$. \end{prop}

We can conclude that in the same pair of countable models of set theory, the internal categories $SET$ are not MacLane equivalent.



==> sections2022/computably-tdlc.tex <==
\section{Computably t.d.l.c.\ groups}
This talk was   mainly based on the 2022 preprint Melnikov and  N., computably t.d.l.\ groups, arxiv 2204.09878.
Recall that in this post, topological groups are always    countably  based.  Recall that a   topological group $G$ is t.d.l.c.\ if its underlying  topology is totally disconnected and locally compact. Van Dantzig 1936 proved that $G$ has an open compact subgroup, and hence a nbhd basis of 1 of compact open subgroups. This implies that such groups are homeomorphic to closed subgroups of $S_\infty$ (via the left action on the compact open cosets). 

Examples of t.d.l.c.\ groups include \bi \item algebraic groups over local fields, such as $SL_n(\QQ_p)$, \item the automorphism groups of countable locally finite graphs, such as $\Aut(T_d)$, and also \item the split extension $\ZZ \ltimes \QQ$ with the continuous action of $\ZZ$ given by $\la z,x \ra \to p^{-z}x$. \ei Note that there are 3 general types of topological subgroups: 

\bc compact open $\Rightarrow$  open $\Rightarrow$ closed.\ec
There are only countably  many compact open subgroups. The closed subgroups form a (easily uncountable) compact space known as the Chabauty space.

How do we present a t.d.l.c.\ group in a ``computable" way? The examples above seem computable in an ad-hoc way, but what is a general notion? 
We introduce two main types of computable presentation: Baire type (B) and meet groupoid type (M) , and show their equivalence. 

\n \emph{Presentations of type (B).} We start from this well-known fact. Baire space $\+ N = \NN^\NN$ is equipped with the usual product topology where $\NN$ carries the discrete topology. It can be thought of as  $[\NN^*]$, i.e.\ the set of paths on an always  infinitely branching tree. 
\begin{fact}[see \cite{Kechris:95}, Thm I.7.8] Each separable 0-dimensional  space is homeomorphic to a closed subspace $\+ S$ of Baire space $\+ N = [\NN^*]$, i.e.\ the set of paths on an always  infinitely branching tree $T$.  \end{fact}
Write $[\sss]_T = \{f \in [T] \colon \sss \prec f\}$ for the cone based at a string $\sss$. Clearly, the t.d.l.c.\ spaces are given by trees $T$ such that along any path, the tree eventually gets finitely branching.  In other words, for each $f \in [T]$ there is $\sss \prec f$ such that $[\sss]_T $ is compact. 

Every t.d.l.c.\ group  $(G, \cdot, {}^{-1})$ has a presentation \bc $(\+ S, \mathrm{Mult}, \mathrm{Inv})$ \ec such that  the operations $ \mathrm{Mult} \colon \+ S \times \+ S \to \+ S$ and $\mathrm{Inv} \colon \+ S \to \+ S$ are continuous. 

\n \emph{Presentations of type (M).}  We present $G$ by its meet groupoid $\+ W(G)$ as defined in Section~\ref{ss: mg}; this is a  countable structure of approximations to elements of $G$,   the compact open cosets    with partial product, inverse, and intersection operation. As in Section~\ref{ss: mg} we have a duality   

class of t.d.l.c.\ groups $\xymatrix{{\mathcal C} \ar@/^/^{\+ W}[r]& {\mathcal D}\ar@/^/^{ \+ G}[l] }=$ a certain Borel class of meet groupoids. 


%\subsection{ Motivation for  studying  computable presentations of t.d.l.c.\ groups $G$}
%
%\begin{enumerate} 
%\item Most examples, including all the ones given above,  appear to be computable in an ad-hoc way. This suggests that a  general framework is needed.
% \item computability notions have been defined for subclasses: the discrete ( in the 1950s) and, lesser known,  the profinite  (in the 1980s) groups. We want to unify these to a concept that works for t.d.l.c.\ groups in general
%
%\item we want to assert in a precise way whether objects associated to $G$ are computable: the modular and the scale functions, and also (if $G$ is compactly generated) the Cayley-Abels graphs. 
%\end{enumerate}
%
% Here's a brief overview of  the computable setting; detail will follow below. 
%
%\n \emph{Type (B)} We suppose that the domain of $G$ is the set of paths $[T]$ on a tree $T \sub \NN^*$, We will define computably locally compact trees $T$, which are the ones where  $[T]$ is locally compact in an effective way. The operations of $G$ are computable on $[T]$ in a sense to be defined 
%
%\n \emph{Type (M)} We  introduce a ``concrete" version $\+ W_{\text{comp}}(G)$ of the meet groupoid of $G$, where the domain doesn't consists of actual compact open cosets, but rather, natural numbers encoding them.  Note that each compact open set $A \sub [T]$ is a finite union of cones: we have $A = \bigcup_{\sss \in F} [\sss]_T$ for some finite set $F \sub T$. Assuming a computable  bijection $\NN^* \to \NN$ (e.g. given by the prime number decomposition), we can encode $F$ by a single natural number.  
%, we can recognize whether a compact open set $A$ is a coset, a subgroup, etc.
%
%
%\subsection{Type (B)}
%
%\subsection{Type (M)}
% \begin{definition}[Haar computable meet groupoids] \label{def:comp_meet_groupoid} A meet groupoid $\+ W$ is called \emph{Haar computable}~if 
%\bi \item[(a)]  its  domain is a computable subset $D$ of $\NN$; 
%
%\item[(b)] the   groupoid and meet operations    are computable; in particular, the relation $\{ \la x,y \ra\colon \, x,y \in S \lland x\cdot y \text{ is defined}\}$   is computable;
% 
% \item[(c)]     the partial function with domain contained in  $D \times D$ sending  a pair of subgroups $U, V\in \+ W $ to $|U:U\cap V|$ is   computable.   \ei
%    \end{definition}
%  Here   $|U \colon U \cap V|$  is  defined abstractly as the number of left, or equivalently right, cosets of $U \cap V$ contained in $U$; we require implicitly that this number is always finite.  Note that by  (b), the partial order induced by the meet semilattice structure of $\+ W$  is computable. Also, (b) implies that being a subgroup is decidable when viewed as a property of elements of the domain  $S$; this is used in (c). 
%  
%  \begin{definition}  A t.d.l.c.\ group $G$ has a computable presentation of type (M) if $\+ W(G) \cong M$ for a Haar computable meet groupoid $M$.\end{definition}
%  
%  \subsection{Equivalence of type (B)  and type (M)}
%  \begin{theorem} The operations $\+ W_{\text{comp}}$ and $\+ G$ exchange    presentations of type (B) and (M) for the same group. \end{theorem}
  
  
  
  
  
  
  
  
  

